Phone2Proc: Bringing Robust Robots Into Our Chaotic World

Training embodied agents in simulation has become mainstream for the embodied AI community. However, these agents often struggle when deployed in the physical world due to their inability to generalize to real-world environments. In this paper, we present Phone2Proc, a method that uses a 10-minute phone scan and conditional procedural generation to create a distribution of training scenes that are semantically similar to the target environment. The generated scenes are conditioned on the wall layout and arrangement of large objects from the scan, while also sampling lighting, clutter, surface textures, and instances of smaller objects with randomized placement and materials. Leveraging just a simple RGB camera, training with Phone2Proc shows massive improvements from 34.7% to 70.7% success rate in sim-to-real ObjectNav performance across a test suite of over 200 trials in diverse real-world environments, including homes, offices, and RoboTHOR. Furthermore, Phone2Proc's diverse distribution of generated scenes makes agents remarkably robust to changes in the real world, such as human movement, object rearrangement, lighting changes, or clutter.

==> extra_02_intro1.tex <==

A large body of research in Embodied AI has focused on using visual simulators~\cite{Kolve2017AI2THORAI,Savva2019HabitatAP,Xia2018GibsonER} to train embodied agent policies with the intention of transferring these policies onto robots in the physical world. Simulators offer several benefits, including the ability to run experiments in parallel at a fraction of the cost of acquiring multiple robots, reproducibility of experiments, accessibility to the broader community, and safety of the workplace.

While agents within these simulated worlds have been getting more capable each year, progress on deploying these policies onto physical robots has been slower. Firstly very few works in Embodied AI measure real world performance owing to the challenges and cost of running real world experiments; the works that do test their models on physical robots tend to either show just qualitative results~\cite{Partsey2022IsMN,chaplot2020learning,Zhu2017TargetdrivenVN}, report real world results on a single environment~\cite{Kadian2020Sim2RealPD,deitke2020robothor} or perform few trials~\cite{Chaplot2020ObjectGN,Gupta2017CognitiveMA,Hirose2019DeepVM}. Secondly, policies trained in simulation that leverage localization sensors for agent location and pose and target location~\cite{chaplot2020learning, Chaplot2020ObjectGN} require expensive real world sensors like LiDAR and do not perform as well in the real world in the absence of perfect sensing. Thirdly, models trained on small sets of simulated environments already struggle with generalizing to new unseen target scenes in simulation; the additional hop from simulation to real causes the target observations to be far out-of-domain which leads to poor performance~\cite{deitke2020robothor}.

In practice, physical robots must not only be far more effective and efficient at their tasks than they currently are, but they must also be able to work in realistic environments. The physical scenes that are typically used to measure real world performance tend to be static and clutter free. In reality, physical spaces such as houses have objects that keep getting displaced, furniture that may shift position, humans that keep moving around as the robot navigates, clutter and messy spaces and lighting that keeps changing as the day transitions to night and lights go on and off. Although we are making good progress in simulation, we are still far away from producing performant, robust, and resilient physical agents. 


In this work we present \methodName, a method that takes a big leap towards this goal and produces embodied AI agents that work effectively and robustly within a desired physical world (Figure~\ref{fig:teaser}). \methodName\ uses Apple’s freely available RoomPlan API to quickly scan a real world target environment using an iPhone and produce a template of the scene that provides wall layouts, doors and windows and 3D placements of large objects in the scene like couches and tables. \methodName\ then leverages the power of ProcTHOR~\cite{deitke2022procthor} to convert this scan into a fully interactive rich simulated environment. Using ProcTHOR allows us to easily add new objects into this world, randomize their placements and vary materials, lighting and textures in the scene. This results in a large but targeted set of simulated training environments which are used to train embodied agents for transfer and evaluation in the real world.

We use \methodName\ to produce policies for object goal navigation and deploy them onto a LocoBot robot in the physical world. We perform large scale evaluations with 234 episodes within 5 diverse physical environments, a 3 room apartment, a large 6 room apartment, a test scene in RoboTHOR-real, a conference room and a cafeteria -- which represents one of the largest and most diverse real world studies of sim-to-real navigation agents. In each of the 5 spaces, we find that \methodName\ hugely outperforms the state of the art embodied AI model built with ProcTHOR~\cite{deitke2022procthor}, improving on average the success rate from 34.7\% to 70.7\%. We find that our robot explores the scene efficiently and is effective at locating and navigating to objects of interest, in spite of encountering clutter, lighting changes, shifts in furniture and even humans moving around. These strong navigation results in the real world are obtained in spite of using an \textbf{RGB-only} camera, \textbf{no depth} or LiDAR sensors, \textbf{no localization} sensors, and \textbf{no explicit mapping} components. 


\noindent In summary, our contributions include: (1) \methodName, an easy and highly effective method to train embodied agents for the real world using a phone and leveraging the flexibility of ProcTHOR, (2) Large scale real world robotics experiments with 234 trials showing huge improvements for \methodName\ over the present state of the art model in simulation, and (3) Demonstrating the robustness of \methodName\ across changes in lighting, rearrangements, clutter, humans and other variations one may expect in our chaotic real worlds.


==> extras.tex <==

Truong \etal\cite{Truong2022RethinkingSL} compares the correlation of performance of models in simulation against real world. sim2real (with exact sim version actually) but uses depth and distance + heading to goal. find that higher simulation
fidelity does not enable learning better high-level visual navigation policies. \kiana{mention this in experiment too?}
\cite{Kadian2020Sim2RealPD}  sim2real but in super simplistic setting (blocks and stufF) and for pointnav %
\cite{Bigazzi2021OutOT} only 5 examples in RW, uses agent pose and rgbd and is for pointnav%
\cite{Sadek2022AnIE} show good generalization of sim2real but only for pointnav which is not realistic, %
\cite{Dugas2022NavDreamsTC} moving people, not for object nav 
\cite{Truong2021BiDirectionalDA} domain adaptation for sim2real gap but with simplistic envs for pointnav
\cite{Anderson2020SimtoRealTF} for vision and language
\cite{Kadian2019AreWM} simple env wih blocks and for the task of pointnav






\begin{figure}[tp]
    \centering
    \includegraphics[width=20pc]{assets/result_figure.pdf}
    \caption{Results for \methodName vs ProcTHOR baseline in a variety of real environments. Each number represents fifteen trajectories - five objects from three starting locations. \ani{Try bar graph or some way to make this much larger.}}
    \label{fig:four_env_results}
\end{figure}

In roboTHOR, we additionally trained a model in the simulated reconstruction of the test scene, to determine and compare to a theoretical upper bound on performance. This model performs well (as expected) when the scene remains static, but is brittle when naturalistic changes are introduced. \methodName is more robust to these changes both in real and simulated episodes.

\begin{table}[tp]
\footnotesize
\setlength{\tabcolsep}{2pt}
	\centering
\hfill
	\begin{tabular}{l|c|c}
    Model  & ObjectNav in Sim  & ObjectNav in Real \tabularnewline
\toprule 
Habitat\cite{Ramakrishnan2021HabitatMatterport3D}  - Limited Set & 0.0 & 0.0 \tabularnewline
\midrule
\methodName - Limited Set & 88.8 & 77.8 \tabularnewline 
\midrule
\midrule
ProcTHOR \cite{deitke2022procthor} & 40.0 & 26.6 \tabularnewline
\midrule
Reconstructed Simulation\cite{deitke2020robothor}& 100 & 73.3 \tabularnewline
\midrule
\methodName & 60.0 & 73.3\tabularnewline
\bottomrule

	\end{tabular}
\hfill 
	\vspace{0cm}
	\caption{Despite our efforts tuning camera parameters, we were not able to get the model trained on Habitat off the ground. However, this is consistent with the findings by Chaplot \etal\cite{Chaplot2020ObjectGN}: ``End-to-end learning-based policies failed consistently in the real-world due to the visual domain gap between simulation environments and the real-world." The ProcTHOR baseline achieves some success and as expected, the reconstruction model performs well in sim and real, similar to \methodName. However, the reconstruction very labor-intensive to create and is brittle to scene changes where \methodName is not (see Fig. \ref{fig:fragility}). \rose{not sure I like the habitat stuff here  - could move to exp. but if someone's going to be upset about the zeros in the table there should be something about it in the caption} 
	}
	\label{table:robothor_results}
\end{table}

Dugas \etal\cite{Dugas2022NavDreamsTC} introduce a dataset for building models robust to moving people. 


\cite{Kang2021MultiRobotDR} hierarchically integrated models 
\cite{Kahn2018ComposableAP} train on simulation, gather data on real, autonomously train, focused on control



---------------






